Quadraxial metamaterial

We study the dispersion of electromagnetic waves in a spatially dispersive metamaterial with Lorentz-like dependence of principal permittivity tensor components on the respective components of the wave vector performing the analysis of isofrequency contours. The considered permittivity tensor describes triple non-connected wire medium. It is demonstrated that the metamaterial has four optic axes in the frequency range below artificial plasma frequency. The directions of the optical axes do not depend on frequency and coincide with the diagonals of quadrants. The metamaterial supports two propagating electromagnetic waves in all directions of space except the directions of axes. The conical refraction effect is observed for all four optic axes both below and above artificial plasma frequency where the metamaterial supports five propagating waves in most of the directions.

==> eqs-ncwm.tex <==
\section{Equations for TWM}
\begin{align}
	C&\left(k_0, k_{x}, k_{y}, k_{z}, a\right)= \nonumber \\ =&\frac{\eta\left(k_0^{2}-k_{z}^{2}\right)}{2 j k_0 a}\left[\frac{1}{k_{0x}^{(0)}} \frac{\sin k_{0x}^{(0)} a}{\cos k_{0x}^{(0)} a-\cos k_{x} a}+\right. \nonumber \\
	&+\sum_{n \neq 0}\left(\frac{1}{k_{0x}^{(n)}} \frac{\sin k_{0x}^{(n)} a}{\cos k_{0x}^{(n)} a-\cos k_{x} a}-\frac{a}{2 \pi|n|}\right)+ \nonumber \\
	&\left.+\frac{a}{\pi}\left(\log \frac{\sqrt{k_0^{2}-k_{z}^{2}} a}{4 \pi}+\gamma\right)+j \frac{a}{2}\right]
\end{align}
where $\eta=\sqrt{\mu_0/\varepsilon_0}$ and
\begin{equation}
	k_{0x}^{(n)}=-j \sqrt{\left(k_{y}+\frac{2 \pi n}{a}\right)^{2}+k_{z}^{2}-k_0^{2}}
\end{equation}

\begin{equation}
	\begin{array}{l}
		\left(C_{x x}-\alpha_{x}^{-1}\right) I_{x}+C_{x y} I_{y}+C_{x z} I_{z}=0 \\
		C_{y x} I_{x}+\left(C_{y y}-\alpha_{y}^{-1}\right) I_{y}+C_{y z} I_{z}=0 \\
		C_{z x} I_{x}+C_{z y} I_{y}+\left(C_{z z}-\alpha_{z}^{-1}\right) I_{z}=0
	\end{array}
\end{equation}

\begin{align}
	&C_{xx}=C\left(k_0, k_{y}, k_{z}, k_{x}, a\right) \nonumber \\
	&C_{yy}=C\left(k_0, k_{x}, -k_{z}, k_{y}, a\right) \nonumber \\
	&C_{zz}=C\left(k_0, k_{x}, k_{y}, k_{z}, a\right) \nonumber \\
	&C_{y x}=j \frac{\eta k_{x} k_{y}}{k_{0z} k_0 a} \frac{\cos \left(k_{z} a / 2\right) \sin \left(k_{0z} a / 2\right)}{\cos k_{z} a-\cos k_{0z} a} e^{-j k_{z} a / 2} \nonumber \\
	&C_{z x}=j \frac{\eta k_{x} k_{z}}{k_{0y} k_0 a} \frac{\cos \left(k_{y} a / 2\right) \sin \left(k_{0y} a / 2\right)}{\cos k_{y} a-\cos k_{0y} a} e^{-j k_{y} a / 2} \nonumber \\
	&C_{z y}=j\frac{\eta k_{y} k_{z}}{k_{0x} k_0 c} \frac{\cos \left(k_{x} a / 2\right) \sin \left(k_{0x} a / 2\right)}{\cos k_{x} a-\cos k_{0x} a}e^{-j k_{x} a / 2} \nonumber \\
	&C_{xy}=C_{yx}e^{jk_za}\quad C_{xz}=C_{zx}e^{jk_ya}\quad C{yz}=C_{zy}e^{jk_xa}
\end{align}
where
\begin{align}
	&k_{0_x} \equiv-j \sqrt{k_{y}^{2}+k_{z}^{2}-k_0^{2}} \nonumber \\
	&k_{0_y} \equiv-j \sqrt{k_{x}^{2}+k_{z}^{2}-k_0^{2}} \nonumber \\
	&k_{0_z} \equiv-j \sqrt{k_{x}^{2}+k_{y}^{2}-k_0^{2}}
\end{align}

\begin{figure}[h]%----------------------------------------FIG
	\begin{minipage}[h]{0.49\linewidth}
		\center{\includegraphics[width=1\textwidth]{fig/isofreq-surf/biax-disp-surf-0_225-eight.png} \\ (a)}
	\end{minipage}
	\hfill
	\begin{minipage}[h]{0.49\linewidth}
		\center{\includegraphics[width=1\textwidth]{fig/isofreq-surf/ncwm-disp-surf-0_1-eight.png} \\ (b)}
	\end{minipage}
	\vfill
	\begin{minipage}[h]{0.49\linewidth}
		\center{\includegraphics[width=1\textwidth]{fig/isofreq-surf/ncwm-disp-surf-1_01kp-eight.png} \\ (c)}
	\end{minipage}
	\hfill
	\begin{minipage}[h]{0.49\linewidth}
		\center{\includegraphics[width=1\textwidth]{fig/isofreq-surf/ncwm-disp-surf-1_01kp-zoom-eight.png} \\ (d)}
	\end{minipage}
	\caption{One eight of the Brillouin zone with the theoretical (according to Eq. \ref{eq:disp-eq}) isofrequency surface (a) for a biaxial media with the permittivity tensor: $\varepsilon_{xx}=1$, $\varepsilon_{yy}=2$ and $\varepsilon_{zz}=4$ (shape of the surface does not change with frequency); (b,c) for the triple wire metamaterial at $\omega a/2\pi c=0.1$ and at $\omega =1.01\omega_p$ respectively. (d) Zoomed plasmonic mode for the triple wire metamaterial at $\omega =1.01\omega_p$ (circled part in subfigure (c)).}
	\label{fig:isofreq-ex}
\end{figure}

Dispersion equation (simplified):
\begin{align}
	&\left(k_0^{2}-k_{x}^{2}\right)\left(k_0^{2}-k_{y}^{2}\right)\left(k_0^{2}-k_{z}^{2}\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right]\times \nonumber \\
	&\times\left[k_0^{2}-k_{p}^{2}-k^{2}\right]\left[k_0^{2}-k_{p}^{2}-k^{2}\right]- \nonumber \\
	&-\left(k_0^{2}-k_{x}^{2}\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right] k_{y}^{2} k_{z}^{2} k_{p}^{4}- \nonumber \\
	&-\left(k_0^{2}-k_{y}^{2}\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right] k_{x}^{2} k_{z}^{2} k_{p}^{4}- \nonumber \\
	&-\left(k_0^{2}-k_{z}^{2}\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right] k_{x}^{2} k_{y}^{2} k_{p}^{4} +2 k_{x}^{2} k_{y}^{2} k_{z}^{2} k_{p}^{6}=0
\end{align}
OR
\begin{align}
	&\left(k_0^{2}-k_{x}^{2}\right)\left(k_0^{2}-k_{y}^{2}\right)\left(k_0^{2}-k_{z}^{2}\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right]^3-  \nonumber \\
	&-\left\{k_0^{2}\left(k_y^2k_z^2 + k_x^2k_z^2 + k_x^2k_y^2\right) - 3k_x^2k_y^2k_z^2\right\}\times \nonumber \\
	&\times\left[k_0^{2}-k_{p}^{2}-k^{2}\right]k_p^4
	+2 k_{x}^{2} k_{y}^{2} k_{z}^{2} k_{p}^{6}=0
\end{align}
OR
\begin{align}
	&\left(k_0^{2}-k_{x}^{2}\right)\left(k_0^{2}-k_{y}^{2}\right)\left(k_0^{2}-k_{z}^{2}\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right]^3- \nonumber \\
	&-\left\{k_0^{2}\left(k_y^2k_z^2 + k_x^2k_z^2 + k_x^2k_y^2\right) - k_x^2k_y^2k_z^2\right\}\times \nonumber \\
	&\times\left[k_0^{2}-k_{p}^{2}-k^{2}\right]k_p^4
	+2\left(k_0^2-k^2\right)k_{x}^{2} k_{y}^{2} k_{z}^{2} k_{p}^{4}=0
\end{align}
OR
\begin{align}
	&\left(k_0^{2}-k_{x}^{2}\right)\left(k_0^{2}-k_{y}^{2}\right)\left(k_0^{2}-k_{z}^{2}\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right]^3-  \nonumber \\
	&-\left(k_y^2k_z^2 + k_x^2k_z^2 + k_x^2k_y^2\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right]k_0^{2}k_p^4+ \nonumber \\
	&+\left(3k_0^2-k_p^2-3k^2\right)k_{x}^{2} k_{y}^{2} k_{z}^{2} k_{p}^{4}=0
\end{align}
OR (without $k_0^2-k^2=0$ sphere)
\begin{align}
	&\left[k_0^2-k_p^2-k^2\right]^3\left(k_0^4+k_x^2k_y^2+k_x^2k_z^2+k_y^2k_z^2\right)+ \nonumber \\
	&\left[k_0^2-k_p^2-k^2\right]\left\{\left(k_x^2+k_y^2\right)\left(k_x^2+k_z^2\right)\left(k_y^2+k_z^2\right)\times\right. \nonumber \\
	& \times\left.\left(k_0^2-2k_p^2-k^2\right)-k_p^4\left(k_x^2k_y^2+k_x^2k_z^2+k_y^2k_z^2\right)\right\}+ \nonumber \\
	&2k_p^4k_x^2k_y^2k_z^2=0
\end{align}

The same equation in the $k_x=k_y$ \textbf{plane}:
\begin{align}
	&\left(k_0^{2}-k_{x}^{2}\right)^2\left(k_0^{2}-k_{z}^{2}\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right]^3-  \nonumber \\
	&-\left(2k_x^2k_z^2 + k_x^4\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right]k_0^{2}k_p^4+ \nonumber \\
	&+\left(3k_0^2-k_p^2-3k^2\right)k_{x}^{4} k_{z}^{2} k_{p}^{4}=0
\end{align}
OR (without $k_0^2-k^2=0$ sphere)
\begin{align}
	&\left[k_0^2-k_p^2-k^2\right]^3\left(k_0^4+k_x^4+2k_x^2k_z^2\right)+ \nonumber \\
	&\left[k_0^2-k_p^2-k^2\right]\left\{2k_x^2\left(k_x^2+k_z^2\right)^2\left(k_0^2-2k_p^2-k^2\right)-\right. \nonumber \\
	& \left.k_p^4\left(k_x^4+2k_x^2k_z^2\right)\right\}+ 2k_p^4k_x^4k_z^2=0
\end{align}

In the $k_z=0$ (or $k_x=0$ or $k_y=0$) \textbf{plane}:
\begin{align}
	&\left(k_0^{2}-k_{x}^{2}\right)\left(k_0^{2}-k_{y}^{2}\right)k_0^{2}\left[k_0^{2}-k_{p}^{2}-k^{2}\right]^3- \nonumber \\
	&-k_x^2k_y^2\left[k_0^{2}-k_{p}^{2}-k^{2}\right]k_0^{2}k_p^4=0
\end{align}
OR
\begin{align}
	&\left[k_0^{2}-k_{p}^{2}-k^{2}\right]\cdot \left\{\left(k_0^{2}-k_{x}^{2}\right)\left(k_0^{2}-k_{y}^{2}\right)\left[k_0^{2}-k_{p}^{2}-k^{2}\right]^2-\right. \nonumber \\
	&\left.-k_x^2k_y^2k_p^4\right\}=0
\end{align}
OR (without $k_0^2-k^2=0$ sphere) in $k_z=0$ plane
\begin{align}
	&\left[k_0^2-k_p^2-k_{xy}^2\right]\Big\{\left[k_0^2-k_p^2-k_{xy}^2\right]^2\left(k_0^4+k_x^2k_y^2\right)+ \nonumber \\
	& \left(k_0^2-2k_p^2-k_{xy}^2\right)k_{xy}^2k_x^2k_y^2-k_p^4k_x^2k_y^2\Big\}=0
\end{align}

Roots (with $\operatorname{grad}f=0$ condition):
\begin{equation}
	\begin{pmatrix}
		k_x\\
		k_y
	\end{pmatrix}=
	\begin{pmatrix}
		\pm\sqrt{k_0^2-k_p^2}\\
		0
	\end{pmatrix}\quad\text{or}\quad
	\begin{pmatrix}
		0\\
		\pm\sqrt{k_0^2-k_p^2}
	\end{pmatrix}
\end{equation}

In the \textbf{diagonal} $k_x=k_y=k_z\equiv k_d$:
\begin{align}
	&\left(k_0^{2}-k_{x}^{2}\right)^3\left[k_0^{2}-k_{p}^{2}-3k_x^{2}\right]^3 -3k_x^4\left[k_0^{2}-k_{p}^{2}-3k_x^{2}\right]k_0^{2}k_p^4+ \nonumber \\
	&+\left(3k_0^2-k_p^2-9k_x^2\right)k_{x}^{6} k_{p}^{4}=0
\end{align}
OR
\begin{align}
	&\cancel{\left(k_0^2 - 3k_x^2\right)}\cdot\left(- k_0^2 + k_p^2 + k_x^2\right)\cdot\nonumber \\
	&\cdot\left(k_0^4 - k_0^2k_p^2 -4k_0^2k_x^2 + 3k_x^4\right)^2=0
\end{align}
Roots:
\begin{equation}
	k_d=\left\{
	\begin{matrix*}[l]
			\pm\sqrt{(k_0^2 - k_p^2)}\\
			\pm\sqrt{\frac{k_0}{3}\left(2k_0 - \sqrt{k_0^2 + 3k_p^2}\right)}\\
			\pm\sqrt{\frac{k_0}{3}\left(2k_0 + \sqrt{k_0^2 + 3k_p^2}\right)}
	\end{matrix*} \right.
\end{equation}
